Surface-like boundaries of hyperbolic groups

We classify the boundaries of hyperbolic groups that have enough quasiconvex codimension-1 surface subgroups with trivial or cyclic intersections.

==> submission version/notations.tex <==

\newenvironment{new}{\color{red}} {}

\newcounter{dummy} \numberwithin{dummy}{section}
\newtheorem{theorem}[dummy]{Theorem}
 
\newtheorem{claim}[dummy]{Claim}
\newtheorem{lemma}[dummy]{Lemma}
\newtheorem{corollary}[dummy]{Corollary}
\newtheorem{fact}[dummy]{Fact}
\let\oldfact\fact
\renewcommand{\fact}{\oldfact\normalfont}

\newtheorem{question}[dummy]{Question}
\let\oldquestion\question
\renewcommand{\question}{\oldquestion\normalfont}


\newtheorem{definition}[dummy]{Definition}
\let\olddefinition\definition
\renewcommand{\definition}{\olddefinition\normalfont}

\newtheorem{remark}[dummy]{Remark}
\let\oldremark\remark
\renewcommand{\remark}{\oldremark\normalfont}

\newtheorem{example}[dummy]{Example}
\let\oldexample\example
\renewcommand{\example}{\oldexample\normalfont}

%operators
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\Stab}{Stab}
\DeclareMathOperator{\compdiam}{comp-diam}
\DeclareMathOperator{\genus}{genus}
\DeclareMathOperator{\girth}{girth}
\DeclareMathOperator{\rgirth}{girth_r}
\DeclareMathOperator{\level}{level}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\RACG}{RACG}
\DeclareMathOperator{\Link}{Link}
\DeclareMathOperator{\Star}{Star}


%general commands
\newcommand{\N}{\mathbb{N}}
\newcommand{\Nnn}{\mathbb{N}_{\ge 0}}
\newcommand{\R}{\mathbb{R}} 
\newcommand{\Rnn}{\mathbb{R}_{\ge 0}}
\newcommand{\ZZ}{\mathbb{Z}} 

\newcommand{\Ttwo}{\mathbb{T}^2}
\newcommand{\RPtwo}{\mathbb{R}P^2}
\newcommand{\Stwo}{\mathbb{S}^2}
\newcommand{\Sone}{\mathbb{S}^1}
\newcommand{\disk}{\mathbb{D}^2}

\newcommand{\modsim}{/\hspace{-.15cm}\sim}


%specific commands
\newcommand{\skeleton}[1]{\mathcal{#1}}
\newcommand{\cycles}[1]{\mathcal{#1}}
\newcommand{\slcx}[1]{\mathbf{#1}}
\newcommand{\infinitorus}{\mathbb{S}_{\infty}}
\newcommand{\singular}[1]{\mathcal{#1}}
\newcommand{\sided}[1]{\overrightarrow{#1}}
\newcommand{\sidedop}[1]{\overleftarrow{#1}}
\newcommand{\cl}[1]{\overline{#1}}
\newcommand{\SL}[1]{\mathcal{#1}}
\newcommand{\Cells}[1]{\mathcal{#1}}
\newcommand{\embedsin}{\hookrightarrow}
\newcommand{\organism}{organism\xspace}
\newcommand{\mitosis}{mitosis\xspace}
\newcommand{\invlim}{\varprojlim}


\newcommand{\hs}[1]{\overrightarrow{\mathfrak{#1}}}
\newcommand{\hyp}[1]{\mathfrak{#1}}
\newcommand{\sidesof}{\leftthreetimes}
\newcommand{\actson}{\curvearrowright}
\newcommand{\nbd}[1]{\mathcal{U}_{#1}}
\newcommand{\homeo}{\cong}



\newcommand{\editA}[1]{{\color{black} {#1}}}
